Breaking the TDD Flow for Over-the-Air Phase Synchronization in Distributed Antenna Systems

Phase synchronization between distributed antenna arrays requires measurements that break the standard time-division duplex (TDD) operation. We present a feasibility study on implementing such synchronization and analyze its impact on the quality of service. Considering two antenna arrays with independent local oscillators (LOs), we propose a modified TDD flow to accommodate the transmission of phase synchronization signals, formulate the phase estimation and compensation problem, and derive the achievable downlink spectral efficiency (SE). Numerical results show that frequent re-estimation of the interarray phase disparity is essential for maximizing SE in systems with low-quality LOs. Furthermore, applying a Kalman filter for phase tracking substantially improves the SE, especially if phase estimation errors are large compared to LOs phase drifts.

==> acronym.tex <==
% glossaries
\usepackage[toc,acronym,nonumberlist,nopostdot]{glossaries}
\makeatletter
%% patch first occurence of "\@gls@link[#1]{#2}{\@glo@text}", as this is the one for \glsused{#2}
\patchcmd{\@gls@}
  {\@gls@link[#1]{#2}{\@glo@text}}
  {\@gls@link[#1,hyper=false]{#2}{\@glo@text}}
  {}{}

  \patchcmd{\@glspl@}
  {\@gls@link[#1]{#2}{\@glo@text}}
  {\@gls@link[#1,hyper=false]{#2}{\@glo@text}}
  {}{}

  \patchcmd{\@Gls@}
  {\@gls@link[#1]{#2}}
  {\@gls@link[#1,hyper=false]{#2}}
  {}{}

\patchcmd{\@GLS@}
  {\@gls@link[#1]{#2}{\MakeUppercase{\@glo@text}}}
  {\@gls@link[#1,hyper=false]{#2}{\MakeUppercase{\@glo@text}}}
  {}{}
\makeatother


\newacronym{IoT}{IoT}{Internet of Things}
\newacronym{MAC}{MAC}{multiple access channel}
\newacronym{AWGN}{AWGN}{additive white Gaussian noise}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{SINR}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{AP}{AP}{access point}
\newacronym{UE}{UE}{user equipment}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{OFDM}{OFDM}{orthogonal frequency division multiplexing}
\newacronym{TDD}{TDD}{time-division duplexing}
\newacronym{RF}{RF}{radio frequency}
\newacronym{LO}{LO}{local oscillator}
\newacronym{IID}{IID}{independent and identically distributed}
\newacronym{MMSE}{MMSE}{minimum mean squared error}
\newacronym{LMMSE}{LMMSE}{linear minimum mean squared error}
\newacronym{MSE}{MSE}{mean squared error}
\newacronym{CP}{CP}{cyclic prefix}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{IDFT}{IDFT}{inverse discrete Fourier transform}
\newacronym{PN}{PN}{phase noise}
\newacronym{CPE}{CPE}{common phase error}
\newacronym{ICI}{ICI}{inter-carrier interference}
\newacronym{ISI}{ISI}{inter-symbol interference}
\newacronym{IUI}{IUI}{inter-user interference}
\newacronym{SE}{SE}{spectral efficiency}
\newacronym{UatF}{UatF}{use-and-then-forget}
\newacronym{UL}{UL}{uplink}
\newacronym{DL}{DL}{downlink}
\newacronym{iid}{i.i.d.}{independent and identically distributed}

\newacronym{PDF}{PDF}{probability density function}
\newacronym{CDF}{CDF}{cumulative distribution function}
\newacronym{MR}{MR}{maximum ratio}
\newacronym{ZF}{ZF}{zero-forcing}
\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
